Estimating populational-average hazard ratios in the presence of unmeasured confounding

The Cox regression model and its associated hazard ratio (HR) are frequently used for summarizing the effect of treatments on time to event outcomes. However, the HR's interpretation strongly depends on the assumed underlying survival model. The challenge of interpreting the HR has been the focus of a number of recent works. Besides, several alternative measures have been proposed in order to deal with these concerns. The marginal Cox regression models include an identifiable hazard ratio without individual but populational causal interpretation. In this work, we study the properties of one particular marginal Cox regression model and consider its estimation in the presence of omitted confounder. We prove the large sample consistency of an estimation score which allows non-binary treatments. Our Monte Carlo simulations suggest that finite sample behavior of the procedure is adequate. The studied estimator is more robust than its competitors for weak instruments although it is slightly more biased for large effects of the treatment. The practical use of the presented techniques is illustrated through a real practical example using data from the vascular quality initiative registry. The used R code is provided as Supplementary Material.

==> Bibliography.tex <==
@article{andersen82,
author = "Andersen, P. K. and Gill, R. D.",
journal = "Annals of Statistics",
number = "4",
pages = "1100--1120",
title = "Cox's Regression Model for Counting Processes: A Large Sample Study",
volume = "10",
year = "1982"
}

@book{cox87,
author = {Cox, B. and Blaxter, M. and Buckle, A. and Fenner, N. and Golding, J. and Gore, M. and Huppert, F. and Nickson, J. and  Roth, S.M. and Stark, J. and Wadsworth, M. E. J. and Whichelow, M.},
 title = {The health and lifestyle survey. Preliminary report of a nationwide survey of the physical and mental health, attitudes and lifestyle of a random sample of 9,003 British adults},
 year = {1987},
 publisher = {Health Promotion Research Trust},
} 

@incollection{wienke10,
title = "Frailty models in survival analysis",
author = "A Wienke",
publisher = " Chapman \& Hall/CRC Biostatistics Series",
address = "Florida",
year = "2010",
}

@article {hernan06,
author = {Hern\'an, M.A. and Robins, J.M.},
title = {Instruments for causal inference: an epidemioligist's dream?},
journal = {Epidemiology},
volume = {17},
number = {4},
pages = {360--372},
keywords = {Additive hazards model, Instrumental variable, Survival analysis, Two-stage least squares estimation},
year = {2006},
}

@article{angrist96,
author = {J.D. Angrist and G.W. Imbens and D. B. Rubin},
journal = {Journal of the American Statistical Association},
number = {434},
pages = {444--455},
title = {Identification of Causal Effects Using Instrumental Variables},
volume = {91},
year = {1996},
}

@book{pearl00,
 author = {Pearl, J.},
 title = {Causality: Models, Reasoning, and Inference},
 year = {2000},
 publisher = {Cambridge University Press},
 address = {New York, NY, USA},
} 

@manual{survival,
author = {T. Therneau}, 
year = {2015}, 
title = {A Package for Survival Analysis in {S} and {R}}, 
note = {R package version 2.38}, 
url = { https://CRAN.R-project.org/package=survival},
}

@article{stute95,
author = {W. Stute},
title = {The statistical analysis of {K}aplan-{M}eier integrals},
journal = {Analysis of Censored Data, IMS Lecture Notes - Monograph Series},
volume = {27},
pages = {231-254},
year  = {1995},
}

@article{hanley82,
	Author = {Hanley, J.A. and McNeil, B.J.},
	Date-Modified = {2019-10-24 02:32:30 +0000},
	Journal = {Radiology},
	Pages = {29-36},
	Title = {The meaning and use of the area under a receiver operating characteristic ({ROC}) curve},
	Volume = {143},
	Year = {1982}}

@article{kaplan58,
 author = {E.L. Kaplan and P. Meier},
 journal = {Journal of the American Statistical Association},
 number = {282},
 pages = {457--481},
 title = {Nonparametric Estimation from Incomplete Observations},
 volume = {53},
 year = {1958}
}

@article{cox72,
 author = {D. R. Cox},
 journal = {Journal of the Royal Statistical Society. Series B (Methodological)},
 number = {2},
 pages = {187--220},
 title = {Regression Models and Life-Tables},
 volume = {34},
 year = {1972}
}

@article{tan06,
author = {Z. Tan},
title = {Regression and Weighting Methods for Causal Inference Using Instrumental Variables},
journal = {Journal of the American Statistical Association},
volume = {101},
number = {476},
pages = {1607-1618},
year  = {2006},
}

@article{wang18,
author = {Wang, L. and Tchetgen Tchetgen, E.},
title = {Bounded, efficient and multiply robust estimation of average treatment effects using instrumental variables},
journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
volume = {80},
number = {3},
pages = {531-550},
year = {2018}
}


@article{xu00,
    author = {Xu, R. and O'Quigley, J.},
    title = "{Estimating average regression effect under non-proportional hazards}",
    journal = {Biostatistics},
    volume = {1},
    number = {4},
    pages = {423-439},
    year = {2000},
}

@article{monni19,
title = "Measuring Survival Benefit in Health Technology Assessment in the Presence of Nonproportional Hazards",
journal = "Value in Health",
volume = "22",
number = "4",
pages = "431 - 438",
year = "2019",
author = "G. Monnickendam and M. Zhu and J. McKendrick and Y. Su",
}

@article{royston19,
author = {P. Royston and M.K. Parmar},
title= {Restricted mean survival time: an alternative to the hazard ratio for the design and analysis of randomized trials with a time-to-event outcome},
journal= {BMC Medical Research Methodology},
volume= {13}, 
number= {152},
year= {2013},
}

@article{fried16,
author = {Fried, T.R.},
title = {Shared Decision Making--Finding the Sweet Spot},
journal = {New England Journal of Medicine},
volume = {374},
number = {2},
pages = {104-106},
year = {2016},
}


@article{aalen15,
author="Aalen, O.O.
and Cook, Richard J.
and R{\o}ysland, Kjetil",
title="Does {C}ox analysis of a randomized survival study yield a causal treatment effect?",
journal="Lifetime Data Analysis",
year="2015",
volume="21",
number="4",
pages="579--593",
}

@article{camblor17,
author = {Mart\'inez-Camblor, P. and MacKenzie, T.A. and Staiger, D.O. and Goodney, P.P and O'Malley, A.J.},
title = {Adjusting for bias introduced by instrumental variable estimation in the Cox proportional hazards model},
journal = {Biostatistics},
volume = {20},
number = {1},
pages = {80-96},
year = {2019},
}

@article{camblor20a,
author = {Mart\'inez-Camblor, P. and MacKenzie, T.A. and Staiger, D.O. and Goodney, P.P and O'Malley, A.J.},
title = {Summarizing causal differences in survival curves in the presence of unmeasured confounding},
journal = {International Journal of Biostatistics},
volume = {xx},
number = {x},
pages = {xx-xx},
year = {2020},
}

@article{camblor20,
author = {Mart\'inez-Camblor, P. and MacKenzie, T.A. and O'Malley, A.J.},
title = {Generalizing hazard ratios for mis-specified {C}ox regression models},
journal = {xxxxx},
volume = {xx},
number = {x},
pages = {xx-xx},
year = {2020},
}








@article{hernan01,
author = {M.A Hern\'an and B. Brumback and J.M. Robins},
title = {Marginal Structural Models to Estimate the Joint Causal Effect of Nonrandomized Treatments},
journal = {Journal of the American Statistical Association},
volume = {96},
number = {454},
pages = {440-448},
year  = {2001},
}












@article{camblor18,
author = {Mart\'inez-Camblor, P. and MacKenzie, T.A. and Staiger, D.O. and Goodney, P.P. and O'Malley, A.J.},
title = {An instrumental variable procedure for estimating {C}ox models with non-proportional hazards in the presence of unmeasured confounding},
journal = {Journal of the Royal Statistical Society: Series C (Applied Statistics)},
volume = {68},
number = {4},
pages = {985-1005},
year = {2019},
}


@article{brott16,
author = {Brott, T.G. and Howard, G. and Roubin, G.S. and Meschia, J.F. and Mackey, A. and Brooks, W. and Moore, W.S. and Hill, M.D. and Mantese, V.A. and Clark, W.M. and Timaran, C.H. and Heck, D. and Leimgruber, P.P. and Sheffet, Alice J. and Howard, Virginia J. and Chaturvedi, Seemant and Lal, Brajesh K. and Voeks, Jenifer H. and Hobson, Robert W. II},
title = {Long-Term Results of Stenting versus Endarterectomy for Carotid-Artery Stenosis},
journal = {New England Journal of Medicine},
volume = {374},
number = {11},
pages = {1021-1031},
year = {2016},
}

@article{rosenfield16,
author = {Rosenfield, K. and Matsumura, J.S. and Chaturvedi, S. and Riles, T. and Ansel, G.M. and Metzger, D.C. and Wechsler, L. and Jaff, M.R. and Gray, W.},
title = {Randomized Trial of Stent versus Surgery for Asymptomatic Carotid Stenosis},
journal = {New England Journal of Medicine},
volume = {374},
number = {11},
pages = {1011-1020},
year = {2016},
}


@article{anderson05,
title = "Origins of the limited information maximum likelihood and two-stage least squares estimators ",
journal = "Journal of Econometrics ",
volume = "127",
number = "1",
pages = "1--16",
year = "2005",
author = "T.W. Anderson",
}

@article{martens06,
Author = {Martens, E.P. and Pestman, W.R. and  de Boer, A. and Belitser, S.V. and  Klungel, O.H.},
Journal = {Epidemiology},
Number = {3},
Pages = {261--267},
Publisher = {Elsevier},
Title = {Instrumental Variables: Application and Limitations},
Volume = {17},
Year = {2006}}

@article{pearl95,
author = {Pearl, J.},
title = {Causal diagrams for empirical research},
journal = {Biometrika},
volume = {82},
number = {4},
pages = {669--688},
year = {1995},
}

@article{terza08,
author = {Terza, J.V. and Bradford, W.D. and Dismuke, C.E.},
title = {The use of linear instrumental variables methods in health services research and health economics: a cautionary note},
journal = { Health Research and Educational Trust},
volume = {43},
number = {3},
pages = {1102--1120},
year = {2008}}



@inbook {kalbfleisch02,
author = {Kalbfleisch, J.D. and Prentice, R.L.},
publisher = {John Wiley \& Sons, Inc.},
isbn = {9781118032985},
pages = { },
title = {The statistical analysis of failure time data},
year = {2002},
}

@inbook {greene03,
title = {Econometric analysis},
author = {Greene, W.H. and Zhang, G.},
publisher = {Prentice Hall, New Jersey, USA},
pages = { },
year = {2003},
}

@article{hausman78,
 author = {J. A. Hausman},
 journal = {Econometrica},
 number = {6},
 pages = {1251-1271},
 title = {Specification Tests in Econometrics},
 volume = {46},
 year = {1978}
}

@article{terza08b,
title = "Two-stage residual inclusion estimation: Addressing endogeneity in health econometric modeling ",
journal = "Journal of Health Economics ",
volume = "27",
number = "3",
pages = "531 - 543",
year = "2008",
author = "J.V. Terza and A. Basu and P.J. Rathouz",
}

@article{normand11,
  Author = {Normand, S.-L.T. and Frank, R.G. and O'Malley, A.J.},
  Title = {Estimating cost-offsets of new medications: Use of new antipsychotics and mental health costs for schizophrenia},
  Journal = {Statistics in Medicine},
  Volume = {30},
  Number = {16},
  Year = {2011},
  Pages = {1971--1988},
}

@article {cai11,
author = {Cai, B. and Small, D.S. and Have, T.R.T.},
title = {Two-stage instrumental variable methods for estimating the causal odds ratio: Analysis of bias},
journal = {Statistics in Medicine},
volume = {30},
number = {15},
issn = {1097-0258},
pages = {1809--1824},
year = {2011},
}

@article{robins91,
author = {J.M.  Robins  and  A.A.  Tsiatis },
title = {Correcting for non-compliance in randomized trials using rank preserving structural failure time models},
journal = {Communications in Statistics - Theory and Methods},
volume = {20},
number = {8},
pages = {2609-2631},
year = {1991},
}

@article {li15,
author = {Li, J. and Fine, J. and Brookhart, A.},
title = {Instrumental variable additive hazards models},
journal = {Biometrics},
volume = {71},
number = {1},
pages = {122--130},
year = {2015},
}

@article {tchetgen15,
author = {Tchetgen Tchetgen,  E.J. and Walter, S. and Vansteelandt, S. and Martinussen, T. and Glymour, M.},
title = {Instrumental variable estimation in a survival context},
journal = { Epidemiology},
volume = {26},
number = {3},
pages = {402--410},
year = {2015},
}

@article {hernan10,
author = {Hern\'an, M.A.},
title = {The hazards of hazard ratios},
journal = {Epidemiology},
volume = {21},
number = {1},
pages = {13--15},
year = {2010},
}

@incollection{heckman85,
title = "Heterogeneity, omitted variable bias, and duration dependence",
author = "G. Chamberlain",
booktitle = "Longitudinal Analysis of Labor Market Data:",
publisher = "Cambridge University Press",
year = "1985",
editor = "James J. Heckman and Burton S. Singer",
address = "Cambridge"
}

@article{gail84,
author = {Gail, M.H. and Wieand, S. and Piantadosi, S.},
title = {Biased estimates of treatment effect in randomized experiments with nonlinear regressions and omitted covariates},
journal = {Biometrika},
volume = {71},
number = {3},
pages = {431--444},
year = {1984},
}

@article{todd12,
title = "Review of case-mix corrected survival curves ",
journal = "The Annals of Thoracic Surgery ",
volume = "93",
number = "5",
pages = "1416 - 1425",
year = "2012",
author = "T.A. MacKenzie and J.R. Brown and D.S. Likosky and Y. Wu and G.L. Grunkemeier"
}


@article {R15,
author = {Schmoor, C. and Schumacher, M.},
title = {Effects of covariate omission and categorization when analysing randomized trials with the {C}ox model},
journal = {Statistics in Medicine},
volume = {16},
number = {3},
pages = {225--237},
year = {1997},
}

@article{todd14,
author="MacKenzie, T.A. and Tosteson, T.D. and Morden, N.E. and Stukel, T.A. and O'Malley, A.J.",
title="Using instrumental variables to estimate a {C}ox's proportional hazards regression subject to additive confounding",
journal="Health Services and Outcomes Research Methodology",
year="2014",
volume="14",
number="1",
pages="54--68",
}

@article{todd16,
author="MacKenzie, T.A. and  L$\o$berg, M. and O'Malley, A.J.",
title="Patient centered hazard ratio estimation using principal stratification weights: application to the {NORCCAP} randomized trial of colorectal cancer screening",
journal="Observational Studies",
year="2016",
volume="2",
number=" ",
pages="29--50",
}

@article {wan,
author = {Wan, Fei and Small, Dylan and Bekelman, Justin E. and Mitra, Nandita},
title = {Bias in estimating the causal hazard ratio when using two-stage instrumental variable methods},
journal = {Statistics in Medicine},
volume = {34},
number = {14},
pages = {2235--2265},
year = {2015},
}


@article {thanasassoulis09,
author = {Thanasassoulis, P. and O'Donnell, T.J.},
title = {Mendelian randomization},
journal = {Journal of American Medical Association},
volume = {301},
number = {22},
pages = {2386--2388},
year = {2009},
}

@article{therneau03,
 author = {Terry M. Therneau and Patricia M. Grambsch and V. Shane Pankratz},
 journal = {Journal of Computational and Graphical Statistics},
 number = {1},
 pages = {156-175},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd., Institute of Mathematical Statistics, Interface Foundation of America]},
 title = {Penalized Survival Models and Frailty},
 volume = {12},
 year = {2003},
}

@article{ripatti00,
 author = {Samuli Ripatti and Juni Palmgren},
 journal = {Biometrics},
 number = {4},
 pages = {1016-1022},
 publisher = {[Wiley, International Biometric Society]},
 title = {Estimation of Multivariate Frailty Models Using Penalized Partial Likelihood},
 volume = {56},
 year = {2000}
}

@article {vaida00,
author = {Vaida, Florin and Xu, Ronghui},
title = {Proportional hazards model with random effects},
journal = {Statistics in Medicine},
volume = {19},
number = {24},
publisher = {John Wiley & Sons, Ltd.},
pages = {3309--3324},
year = {2000},
}

@article{gert92,
 author = {Gert G. Nielsen and Richard D. Gill and Per Kragh Andersen and Thorkild I. A. Sørensen},
 journal = {Scandinavian Journal of Statistics},
 number = {1},
 pages = {25-43},
 publisher = {[Board of the Foundation of the Scandinavian Journal of Statistics, Wiley]},
 title = {A Counting Process Approach to Maximum Likelihood Estimation in Frailty Models},
 volume = {19},
 year = {1992}
}

@article{cox75,
    author = {Cox, D. R.},
    title = "{Partial likelihood}",
    journal = {Biometrika},
    volume = {62},
    number = {2},
    pages = {269-276},
    year = {1975},
}

@article{dabrowska89,
author = "Dabrowska, Dorota M.",
journal = "Annals of Statistics",
number = "3",
pages = "1157--1167",
title = "Uniform Consistency of the Kernel Conditional {K}aplan-{M}eier Estimate",
volume = "17",
year = "1989"
}


@article {wei92,
	Title = {The accelerated failure time model: a useful alternative to the {C}ox regression model in survival analysis},
	Author = {Wei, LJ},
	Number = {14-15},
	Volume = {11},
	Year = {1992},
	Journal = {Statistics in Medicine},
	Pages = {187-1879},
}




@article{wences94,
author = {W.   Gonzalez-Manteiga  and    C.   Cadarso-Suarez },
title = {Asymptotic properties of a generalized {K}aplan-{M}eier estimator with some applications},
journal = {Journal of Nonparametric Statistics},
volume = {4},
number = {1},
pages = {65-78},
year  = {1994},
publisher = {Taylor & Francis},
}


@article{pardo14,
author = {J. C. Pardo-Fernandez and M. X. Rodr\'iguez-\'Alvarez and I. Van Keilegom },
title = {A review on {ROC} curves in the presence of covariates},
journal = {Revstat - Statistical Journal},
volume = {12},
number = {1},
pages = {21-41},
year  = {2014},
}


@article{murphy95,
author = "Murphy, S. A.",
journal = "The Annals of Statistics",
number = "1",
pages = "182--198",
publisher = "The Institute of Mathematical Statistics",
title = "Asymptotic Theory for the Frailty Model",
volume = "23",
year = "1995"
}

@incollection{R24,
title = "Hidden frailty: myths and reality",
pages = " ",
author = "Yashin, A.I. and MAchine, I.A. and  Begun, A.Z. and Vaupel, J.W.",
publisher = "Research Report, Department of Statistics and Demography, Odense University",
year = "2001",
}

@article{hougaard95,
author="Hougaard, P.",
title="Frailty models for survival data",
journal="Lifetime Data Analysis",
year="1995",
volume="1",
number="3",
pages="255--273",
}

@article{platt09,
author = {Platt, Robert W. and Schisterman, Enrique F. and Cole, Stephen R.},
title = {Time-modified Confounding},
journal = {American Journal of Epidemiology},
volume = {170},
number = {6},
pages = {687-694},
year = {2009},
}

@article{robins86,
title = "A new approach to causal inference in mortality studies with a sustained exposure period--application to control of the healthy worker survivor effect",
journal = "Mathematical Modelling",
volume = "7",
number = "9",
pages = "1393--1512",
year = "1986",
author = "J. Robins",
}

@article {gran17,
author = {Gran, Jon Michael and Hoff, Rune and R{\o}ysland, Kjetil and Ledergerber, Bruno and Young, James and Aalen, Odd O.},
title = {Estimating the treatment effect on the treated under time-dependent confounding in an application to the Swiss {HIV} Cohort Study},
journal = {Journal of the Royal Statistical Society: Series C (Applied Statistics)},
volume = {67},
number = {1},
pages = {103-125},
year = {2018},
}

@article{wan17,
title = "A general approach to evaluating the bias of the two-stage instrumental variables estimators",
journal = "Statistics in Medicine,",
volume = "In press",
number = "",
pages = " ",
year = "2018",
author = "Fei Wan and Nandita Mitra and Dylan Small ",
}

@article{aalen15b,
author = {Aalen, Odd O and Valberg, Morten and Grotmol, Tom and Tretli, Steinar},
title = {Understanding variation in disease risk: the elusive concept of frailty},
journal = {International Journal of Epidemiology},
volume = {44},
number = {4},
pages = {1408--1421},
year = {2015},
}

@article {unkel14,
author = {Unkel, Steffen and Farrington, C. Paddy and Whitaker, Heather J. and Pebody, Richard},
title = {Time varying frailty models and the estimation of heterogeneities in transmission of infectious diseases},
journal = {Journal of the Royal Statistical Society: Series C (Applied Statistics)},
volume = {63},
number = {1},
doi = {10.1111/rssc.12033},
pages = {141--158},
year = {2014},
}

@article {goodney11,
	author = {Goodney, Philip P. and Travis, Lori and Lucas, F. Lee and Fillinger, Mark F. and Goodman, David C. and Cronenwett, Jack L. and Stone, David H.},
	title = {Survival After Open Versus Endovascular Thoracic Aortic Aneurysm Repair in an Observational Study of the Medicare Population Clinical Perspective},
	volume = {124},
	number = {24},
	pages = {2661--2669},
	year = {2011},
	journal = {Circulation}}

@article{burne17,
author = {R.M. Burne and M. Abrahamowicz},
title = {Adjustment for time-dependent unmeasured confounders in marginal structural {C}ox models using validation sample data},
journal = {Statistical Methods in Medical Research,},
volume = {In press},
number = {},
pages = {1--20},
year = {2017},
}

@article{barker05,
author="Barker, Peter and Henderson, Robin",
title="Small Sample Bias in the Gamma Frailty Model for Univariate Survival",
journal="Lifetime Data Analysis",
year="2005",
volume="11",
number="2",
pages="265--284",
}

@article{martinussen17,
author = {Martinussen, T. and N{\o}rbo S{\o}rensen, D. and Vansteelandt, S.},
title = {Instrumental variables estimation under a structural {C}ox model},
journal = {Biostatistics},
volume = {20},
number = {1},
pages = {65-79},
year = {2019},
}

@article{rosenbaum83,
author = {Rosenbaum, P.R. and Rubin, D.B.},
title = {The central role of the propensity score in observational studies for causal effects},
journal = {Biometrika},
volume = {70},
number = {1},
pages = {41-55},
year = {1983},
}

@article{rubin74,
author = {Rubin, D.B.},
title = {Estimating causal effects of treatments in randomized and nonrandomized studies},
journal = {Journal of Educational Psychology},
volume = {65},
number = {5},
pages = {688},
year = {1974},
}


















@article{kosorok04,
author = "Kosorok, M.R. and Lee, B.L. and Fine, J.P.",
fjournal = "The Annals of Statistics",
journal = "Ann. Statist.",
number = "4",
pages = "1448--1491",
title = "Robust inference for univariate proportional hazards frailty regression models",
volume = "32",
year = "2004"
}





@article{klungel15,
author = {Klungel, Uddin and de Boer A. and Belitser S.V. and Groenwold R.H. and Roes, K.C.},
title = {Instumental variable analysis in epidemiologic studies: an overview of the estimation methods},
journal = { Pharmaceutica Analytica Acta},
volume = {6},
number = {4},
pages = {1--9},
year = {2015},
}

@article{nieto96,
author = {Nieto, F.J. and Coresh, J.},
title = {Adjusting Survival Curves for Confounders: A Review and a New Method},
journal = {American Journal of Epidemiology},
volume = {143},
number = {10},
pages = {1059-1068},
year = {1996},
}

@article{martinussen13,
author="Martinussen, Torben and Vansteelandt, Stijn",
title="On collapsibility and confounding bias in {C}ox and {A}alen regression models",
journal="Lifetime Data Analysis",
year="2013",
volume="19",
number="3",
pages="279--296",
}

@article{cox58b,
author = "Cox, D. R.",
fjournal = "The Annals of Mathematical Statistics",
journal = "The Annals of Mathematical Statistics",
number = "2",
pages = "357--372",
title = "Some Problems Connected with Statistical Inference",
volume = "29",
year = "1958",
}

@article{james01,
author= " O'Malley, A. J. and Zou, K. H. and Fielding, J. R. and Tempany, C. M.C.",
title= "Bayesian Regression Methodology for Estimating a Receiver Operating Characteristic Curve with Two Radiologic Applications",
journal = "Academic Radiology",
number = "8",
volume = "8",
year = "2001",
pages= "713--725",
}



@article{zhao16,
author = {Zhao, L. and Claggett, B. and Tian, L. and Uno, H. and Pfeffer, M.A. and Solomon, S.D. and Trippa, L. and Wei, L.J.},
title = {On the restricted mean survival time curve in survival analysis},
journal = {Biometrics},
volume = {72},
number = {1},
pages = {215-221},
}


@article{aalen78,
  author = {Aalen, O. O.},
  intrahash = {ce66c5d7a9ef4aca804c6eae7a850772},
  journal = {The Annals of Statistics},
  number = 4,
  pages = {701-726},
  title = {Nonparametric Inference for a Family of Counting Processes},
  volume = 6,
  year = 1978
}

@article{pena93,
title = "Small sample and efficiency results for the Nelson-Aalen estimator",
journal = "Journal of Statistical Planning and Inference",
volume = "37",
number = "2",
pages = "193 - 202",
year = "1993",
author = "Pe\~ na, E. A. and Rohatgi, V. K.",
}

@article{csorgo96,
author = "Csorg\H{o}, S.",
journal = "Annals of Statistics",
month = "12",
number = "6",
pages = "2744--2778",
title = "Universal Gaussian approximations under random censorship",
volume = "24",
year = "1996"
}




@article{camblor17b,
author = {P. Mart\'inez-Camblor},
title ={Fully non-parametric receiver operating characteristic curve estimation for random-effects meta-analysis},
journal = {Statistical Methods in Medical Research},
volume = {26},
number = {1},
pages = {5-20},
year = {2017},

}


@article{kang18,
author = {Kang, H. and Peck, L. and Keele, L.},
title = {Inference for instrumental variables: a randomization inference approach},
journal = {Journal of the Royal Statistical Society: Series A (Statistics in Society)},
volume = {0},
number = {0},
pages = {1--23},
year={2018}

}



@article{staiger96,
author = {D. Staiger and J.H. Stock},
journal = {Econometrica},
number = {3},
pages = {557--586},
title = {Instrumental Variables Regression with Weak Instruments},
volume = {65},
year = {1997}
}



@article {youden50,
author = {Youden, W. J.},
title = {Index for rating diagnostic tests},
journal = {Cancer},
volume = {3},
number = {1},
pages = {32--35},
year = {1950},
}

@article{irwin49,
author= {Irwin, J.O.},
title= {The standard error of an estimate of expectation of life, with special reference to expectation of tumourless life in experiments with mice},
journal= {The Journal of Hygiene},
year= {1949},
volume= {47},
number= {2},
pages= {188--189},
}

@book{van00,
  title={Asymptotic Statistics},
  author={A.W. van der Vaart},
  year={2000},
  place={Cambridge},
  publisher={Cambridge University Press}
}


@article{cote11,
title = "Comparative study of {ROC} regression technique-Applications for the computer-aided diagnostic system in breast cancer detection",
journal = "Computational Statistics \& Data Analysis",
volume = "55",
number = "1",
pages = "888 - 902",
year = "2011",
author = "M. X. Rodr\'iguez-\'Alvarez and P. G. Tahoces and C. Cadarso-Su\'arez and M. J. Lado",
}


@article{cote17,
author = {M. X. Rodr\'iguez-\'Alvarez and J. Roca-Pardi\~ nas and C. Cadarso-Su\'arez and P. G. Tahoces},
title ={Bootstrap-based procedures for inference in nonparametric receiver-operating characteristic curve regression analysis},
journal = {Statistical Methods in Medical Research},
volume = {27},
number = {3},
pages = {740-764},
year = {2018},
}

@article{truthers86,
    author = {Truthers, C.A. and Kalbfleisch, J.D.},
    title = "{Misspecified proportional hazard models}",
    journal = {Biometrika},
    volume = {73},
    number = {2},
    pages = {363-369},
    year = {1986},
}


@article{wang18b,
    title={Learning Causal Hazard Ratio with Endogeneity},
    author={L. Wang and Tchetgen Tchetgen, E. and T. Martinussen and S. Vansteelandt},
    year={2018},
    number={1807.05313},
    journal={arXiv},
    primaryClass={stat.ME}
}


@article{thanassoulis09,
    author = {Thanassoulis, G. and O'Donnell, C.J.},
    title = {Mendelian Randomization: Nature's Randomized Trial in the Pos-Genome Era},
    journal = {JAMA},
    volume = {301},
    number = {22},
    pages = {2386-2388},
    year = {2009},
}

@article{martinussen20,
author = {T. Martinussen and S. Vansteelandt and P.K. Andersen},
title= {Subtleties in the interpretation of hazard contrasts},
journal= {Lifetime Data Analysis},
doi= {https://doi.org/10.1007/s10985-020-09501-5},
pages = {1-23},
year= {2020},
}


@article{austin11,
author = { P. C.   Austin },
title = {An Introduction to Propensity Score Methods for Reducing the Effects of Confounding in Observational Studies},
journal = {Multivariate Behavioral Research},
volume = {46},
number = {3},
pages = {399-424},
year  = {2011},

}


@article{schermerhorn20,
author = {ML. Schermerhorn and P. Liang and J. Eldrup-Jorgensen and JL. Cronenwett  and BW. Nolan and VS. Kashyap and GJ. Wang and RL. Motaganahalli and MB. Malas},
title = {Association of Transcarotid Artery Revascularization vs Transfemoral Carotid Artery Stenting With Stroke or Death Among Patients With Carotid Artery Stenosis}, 
journal= {Journal of the American Medical Association},
year = {2019},
volume = {322},
numer = {23}, 
pages = {2313-2322}
} 


@Book{efron93,
  Title                    = {An Introduction to the Bootstrap},
  Author                   = {B. Efron and R.J. Tibshirani},
  Publisher                = {Chapman \& Hall/CRC},
  Year                     = {1993},
  Address                  = { Boca Raton, Florida, USA},
  Number                   = {57},
  Series                   = {Monographs on Statistics and Applied Probability, }
}

@article{tchentgen15,
author= {E.J. Tchetgen-Tchetgen and S. Walter and S. Vansteelandt and T. Martinussen and M. Glymour},
title=      {Instrumental variable estimation in a survival context},
journal= {Epidemiology}, 
year=     {2015},
volume= {26},
number= {3}, 
pages= {402-410}
}

@article{todd21,
  author = {T.A. MacKenzie and P. Mart\'inez-Camblor and A.J. O'Malley}, 
  title = {Time dependent hazard ratio estimation using instrumental variables without conditioning on an omitted covariate},
  journal = {BMC Medical Research Methodology},
  volume = {21},
  number = {56},
  year = {2021},
  pages = {1-21}
}


